Apply-<x>Mag: One Tool to Support Many Inclusive Design Methods

Doing inclusive design in HCI practice can be labor-intensive, a costly barrier that some companies and HCI practitioners may be unwilling or unable to overcome. Yet, not doing inclusive design is costly too, in the form of UX barriers that disproportionately disadvantage under-served user populations. To address this problem, we introduce Apply-<x>Mag, an LLM-powered tool to support HCI practitioners' work to design their products inclusively to wide ranges of users. Apply-<x>Mag is general, supporting any inclusive design method that can be expressed as <x>Mags (i.e., using attribute ranges and heuristics). It is also effective: Empirical results with researcher and practitioner teams using various combinations of two <x>Mags on 7 products showed Apply-<x>Mag precision averaging 90-99% and recall averaging 82-89%. Further, its environmental costs were reasonable, costing about the same resources as 2-4 ordinary Google searches.

==> Tables/bugcategoryeval2.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{
\textcolor{red}{
\fixme{FAM}{This table may be obsolete as of 8/28}
Bugs raised by human evaluators versus the tool, by category, in
the industry study (Study~2). Counts are the number of bugs flagged in each
category. The tool matches industry practitioners on page-visible categories, misses
post-action categories, and over-reports access/privacy/structure categories.
}}
\label{tab:bug-categories}
\textcolor{red}{
% \tagpdfsetup{table/header-rows={1}}
\begin{tabular}{@{}lllcc@{}}
\toprule
Method & Bug Category & Pattern & Industry practitioners & Tool \\
\midrule
\multirow{6}{*}{SESMag}
  & Unexplained Jargon                 & Matches         & 14 & 11 \\
  & Lack of Action Guidance            & Matches         & 13 & 16 \\
  & Unexplained Data Requirements      & Matches         &  3 &  4 \\
  & Lack of Risk/Consequence Disclosure& Tool misses     &  9 &  1 \\
  & Unstructured Task Information       & Tool over-reports&  5 & 14 \\
  & Assuming Reliable Tech Access      & Tool over-reports&  1 & 11 \\
\midrule
\multirow{5}{*}{GenderMag}
  & Lack of Help/Guidance              & Matches         & 12 & 12 \\
  & Unclear Action Requirements        & Matches         &  7 & 10 \\
  & Privacy Concerns                   & Matches         &  2 &  2 \\
  & Forced Waiting Period              & Tool misses     &  1 &  0 \\
  & Unexpected Screen/Output           & Tool over-reports&  0 &  2 \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/intersectionalresults.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{ll ccc ccc}
\toprule
& & \multicolumn{3}{c}{\textbf{SESMag}} & \multicolumn{3}{c}{\textbf{GenderMag}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
\textbf{Course} & \textbf{Screen} & TP & FP & FN & TP & FP & FN \\
\midrule
\multirow{2}{*}{CS-Math}
  & Homepage & 3 & 0 & 0 & 2 & 0 & 0 \\
  & Modules  & 3 & 0 & 0 & 3 & 0 & 2 \\
\cmidrule(lr){1-8}
\multirow{3}{*}{CS-Arch}
  & Homepage      & 3 & 0 & 0 & 1 & 1 & 0 \\
  & Assig. Des.   & 2 & 1 & 0 & 3 & 0 & 0 \\
  & Assig. Sub.   & 3 & 1 & 1 & 2 & 0 & 0 \\
\midrule
\textbf{Courseware total} & 31 bug reports & \textbf{14} & \textbf{2} & \textbf{1} & \textbf{11} & \textbf{1} & \textbf{2} \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/qrealproductsMetrics.tex <==
\begin{table}[h]
\caption{Precision, recall, and F1 scores by <x>Mag. \textit{Precision} = TP/(TP+FP); \textit{Recall} = TP/(TP+FN); \textit{F1} = 2(Precision$\times{}$Recall)/(Precision+Recall).}
\label{tab:qrealproductsMetrics}
\centering
% \small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lccc@{}}
\toprule
 & \textbf{SESMag} & \textbf{GenderMag} & \textbf{Overall (weighted average)} \\
\midrule
\textbf{Precision} & 97.7\%  & 100\%   & 98.89\% \\
\textbf{Recall}    & 89.4\%  & 75.0\%  & 81.87\% \\
\textbf{F1}        & 93.33\%    & 85.71\%   &  89.36\%  \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/qrealproductsOverall.tex <==
% Shorter table that matches format of qcourseware, just gives overall counts no bisecting counts
\begin{table}[h]
\caption{
Inclusivity bug report totals for real-world products by team, by <x>Mag, same columns as in Table~\ref{tab:qcoursewareOverall}.
In total, the tool found 72 of the 87 true bugs (as per human judgment).
\textcolor{red}{**Full counts of TP/FP/FN by screen can be found in the supplemental documents.**}
}
\label{tab:qrealproductsOverall-Aggregate}
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lccc@{}}
\toprule [1pt] % bolder line
 {} & \multicolumn{3}{c}{\textbf{SESMag}}  \\
\cmidrule(lr){2-4}
\textbf{Product}
      & \makecell[c]{\textbf{Tool matched}\\\textbf{humans (TP)}}
      & \makecell[c]{\textbf{Tool only}\\\textbf{(FP)}}
      & \makecell[c]{\textbf{Tool missed}\\\textbf{(FN)}} \\
\midrule 
\textbf{Digital wallet}        & 13 & 0  & 2  \\
\addlinespace
\textbf{Learning platform}     & 6  & 1  & 1  \\
\addlinespace
\textbf{Municipal services}    & 23 & 0  & 2  \\
\midrule
\midrule
\textbf{SESMag total}
  & \textbf{42} & \textbf{1} & \textbf{5} \\
\midrule [1pt] % bolder line
 {} & \multicolumn{3}{c}{\textbf{GenderMag}}  \\
\cmidrule(lr){2-4}
\textbf{Product}
      & \makecell[c]{\textbf{Tool matched}\\\textbf{humans (TP)}}
      & \makecell[c]{\textbf{Tool only}\\\textbf{(FP)}}
      & \makecell[c]{\textbf{Tool missed}\\\textbf{(FN)}} \\
\midrule 
\textbf{Digital ID-RP}         & 16 & 0  & 7  \\
\textbf{Digital ID-ES}         & 14 & 0  & 3  \\
\midrule 
\midrule 
\textbf{GenderMag total}
  & \textbf{30} & \textbf{0} & \textbf{10} \\
\midrule [1pt] % bolder line
\textbf{Total overall}
  & \textbf{72} & \textbf{1} & \textbf{15} \\
\bottomrule [1pt] % bolder line
\end{tabular}
\end{table}


% Table for supplemental documents, contains the screens

% \begin{table}[h]
% \caption{
% Detailed bug reports for industry products.}
% \label{tab:qrealproductsOverall}
% \centering
% \small
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{@{}llccc@{}}
% \toprule [1pt] % bolder line
%  {} & {} & \multicolumn{3}{c}{\textbf{SESMag}}  \\
% \cmidrule(lr){3-5}
% \textbf{Product} & \textbf{Screen (\#bug reports)}
%       & \makecell[c]{\textbf{Tool matched}\\\textbf{humans (TP)}}
%       & \makecell[c]{\textbf{Tool only}\\\textbf{(FP)}}
%       & \makecell[c]{\textbf{Tool missed}\\\textbf{(FN)}} \\
% \midrule 
% \textbf{Digital wallet}
%   & Whole homepage (5 reports)            & 5 & 0 & 0 \\
%   & Pick a language (6 reports)           & 5 & 0 & 1 \\
%   & Sign in with Google (4 reports)      & 3 & 0 & 1 \\
% \addlinespace
% \textbf{Learning platform}
%   & Select course (3 reports)          & 2 & 0 & 1  \\
%   & Course progress \& certificate (5 reports)            & 4 & 1 & 0  \\
% \addlinespace
% \textbf{Municipal services}
%   & Homepage (5 reports)                 & 5 & 0 & 0  \\  % home-page.png
%   & Create campaign (4 reports)          & 4 & 0 & 0  \\  % create-campaign-options.png
%   & Prepare campaign (4 reports)         & 3 & 0 & 1  \\  % new-campaign-notes.png
%   & Type of campaign (4 reports)         & 3 & 0 & 1  \\  % choose-campaign.png
%   & Campaign type picked (4 reports)     & 4 & 0 & 0  \\  % selected-campaign.png
%   & Campaign duration (4 reports)        & 4 & 0 & 0  \\  % date-campaign.png
% \midrule
% \midrule
% \textbf{SESMag total}
%   & {48 bug reports} & \textbf{42} & \textbf{1} & \textbf{5} \\
% % FAM: consider separating the table
% \midrule [1pt] % bolder line
%  {} & {} & \multicolumn{3}{c}{\textbf{GenderMag}}  \\
% \cmidrule(lr){3-5}
% \textbf{Product} & \textbf{Screen (\#bug reports)}
%       & \makecell[c]{\textbf{Tool matched}\\\textbf{humans (TP)}}
%       & \makecell[c]{\textbf{Tool only}\\\textbf{(FP)}}
%       & \makecell[c]{\textbf{Tool missed}\\\textbf{(FN)}} \\
% \midrule 
% \textbf{Digital ID-RP}
%   & Dashboard (4 reports)                    & 2 & 0 & 2  \\  % image-1.png
%   & Get ID (4 reports)                       & 2 & 0 & 2  \\  % image-16.png
%   & ID pop-up confirmation (3 reports)       & 2 & 0 & 1  \\  % image-22.png
%   & Verify phone/email ID (3 reports)        & 1 & 0 & 2  \\  % image-28.png
%   & Manage virtual ID (3 reports)            & 3 & 0 & 0  \\  % image-39.png
%   & Secure my ID (3 reports)                 & 3 & 0 & 0  \\  % image-41.png
%   & Secure my ID, click submit (3 reports)   & 3 & 0 & 0  \\  % image-42-55.png
% \addlinespace
% \textbf{Digital ID-ES}
%   & Sign in to portal (2 reports)            & 2 & 0 & 0 \\  % image-62.png
%   & Login with VID (3 reports)               & 3 & 0 & 0 \\  % image-63.png
%   & Enter one-time-passcode (4 reports)      & 4 & 0 & 0 \\  % image-73-74-84.png
%   & Request data share consent (6 reports)   & 3 & 0 & 3 \\  % image-76-88.png
%   & Select login mode (2 reports)            & 2 & 0 & 0 \\  % image-91.png
% \midrule 
% \midrule 
% \textbf{GenderMag total}
%   & {40 bug reports} & \textbf{30} & \textbf{0} & \textbf{10} \\
% \midrule [1pt] % bolder line
% \textbf{Total overall}
%   & {88 bug reports} & \textbf{72} & \textbf{1} & \textbf{15} \\
% \bottomrule [1pt] % bolder line
% \end{tabular}
% \end{table}
